Inducing Efficient and Equitable Professional Networks through Link Recommendations

Professional networks are a key determinant of individuals' labor market outcomes. They may also play a role in either exacerbating or ameliorating inequality of opportunity across demographic groups. In a theoretical model of professional network formation, we show that inequality can increase even without exogenous in-group preferences, confirming and complementing existing theoretical literature. Increased inequality emerges from the differential leverage privileged and unprivileged individuals have in forming connections due to their asymmetric ex ante prospects. This is a formalization of a source of inequality in the labor market which has not been previously explored. We next show how inequality-aware platforms may reduce inequality by subsidizing connections, through link recommendations that reduce costs, between privileged and unprivileged individuals. Indeed, mixed-privilege connections turn out to be welfare improving, over all possible equilibria, compared to not recommending links or recommending some smaller fraction of cross-group links. Taken together, these two findings reveal a stark reality: professional networking platforms that fail to foster integration in the link formation process risk reducing the platform's utility to its users and exacerbating existing labor market inequality.

==> archive/eqbm.tex <==
\section{Notes on the Equilibrium Concept}

On 11/8/24 and 11/12/24, we discussed two example scenarios in which the DFPNE solution concept behaves counterintuitively. In the first example, DFPNE \emph{rules out} a certain edge set that we intuitively think ought to be ``stable'' (i.e. the equilibrium concept is too restrictive) and in the other example, the DFPNE condition is satisfied by an edge set that we intuitively think ought \emph{not} to be stable (i.e. the concept is too permissive).

\begin{itemize}
    \item \textbf{Example 1.} This example will involve individuals of \emph{three} exogenous privilege distributions: $g$ (good), $m$ (medium), and $b$ (bad). \pranay{I could not easily think of a way to make this scenario arise with just two distinct privilege levels. Is this a situation that only arises with three or more?}
    % https://q.uiver.app/#q=WzAsMyxbMCwxLCJnIl0sWzIsMSwiYiJdLFsxLDAsIm0iXSxbMCwyLCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMiwiIiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=
    \[\begin{tikzcd}
    	& m \\
    	g && b
    	\arrow[no head, from=2-1, to=1-2]
    	\arrow[dashed, no head, from=2-3, to=1-2]
    \end{tikzcd}\]
    The three individuals receive zero opportunities with probabilities $g_0 < m_0 < b_0$. They receive a surplus of opportunities (i.e. two) with probabilities $g_2 > m_2 > b_2$. We will choose these parameters, along with the edge cost $\gamma$, in such a way that:
    \begin{enumerate}
        \item[(a)] $g$ would prefer to link with just $m$, but only if it has $m$'s undivided attention. If $m$ were to connect with anyone else, $g$ would prefer to drop the link with $m$ altogether.
        \item[(b)] $m$ would prefer to link with both $g$ and $b$ if possible, but if forced to choose at most one, it would prefer to link with $g$ than with $b$.
    \end{enumerate}
    One parameter setting for which this occurs is $(g_0, m_0, b_0) = (b_2, m_2, g_2) = (\varepsilon, 2\varepsilon, 3\varepsilon)$ and $\gamma = \frac{3}{2}\varepsilon^2$ for any strictly positive $\varepsilon < \frac{1}{12}$. In this example, the edge set consisting of a single link between $g$ and $m$ is \emph{not} a DFPNE because $m$ has the option of---in a single step---connecting with $b$, as well. However, it seems as though this edge set should nevertheless be considered ``stable'' because if $m$ were to connect with $b$, it would subsequently lose its more profitable connection with $g$. Therefore, if $m$ were certain this would be the repercussion of connecting with $b$, it should choose to leave things as they are.

    \item \textbf{Example 1.5.} In the previously defined setup with three nodes ($g$, $m$, and $b$), there are no DFPNEs, which seems contrary to intuition.

    \item \textbf{Example 2.} \pranay{Can someone add this? I do not know the details.}
    \end{itemize}
